End-to-End Fast Training of Communication Links Without a Channel Model via Online Meta-Learning

When a channel model is not available, the end-to-end training of encoder and decoder on a fading noisy channel generally requires the repeated use of the channel and of a feedback link. An important limitation of the approach is that training should be generally carried out from scratch for each new channel. To cope with this problem, prior works considered joint training over multiple channels with the aim of finding a single pair of encoder and decoder that works well on a class of channels. In this paper, we propose to obviate the limitations of joint training via meta-learning. The proposed approach is based on a meta-training phase in which the online gradient-based meta-learning of the decoder is coupled with the joint training of the encoder via the transmission of pilots and the use of a feedback link. Accounting for channel variations during the meta-training phase, this work demonstrates the advantages of meta-learning in terms of number of pilots as compared to conventional methods when the feedback link is only available for meta-training and not at run time.

==> meta_training.tex <==
\vspace{-0.52cm}

\section{Fast Training via Meta-Learning} 
\label{sec:meta}

In practice, one is interested in designing encoder parameter $\theta_\text{T}$ and decoder parameter $\theta_\text{R}$ for any new channel $h$ by using a small number of iterations. In this section, we tackle this problem via meta-learning. The key idea is to choose the initialization $\theta^{(0)}$ in Algorithm~\ref{alg:simple_ae} in such a way that a few steps of SGD \eqref{eq:sgd} can yield effective encoder and decoder for \emph{any} channel $h$.

\subsection{Joint Learning}
\label{subsec:meta_setup}
In order to introduce meta-learning, let us first consider the simpler approach of \emph{joint training}. Under joint training, we wish to find a unique solution parameter $\theta$ that works well on all channels in a set $\mathcal{H}=\{ h_k \}_{k=1}^K$ sampled from a given fading distribution. The common model should hence ideally approximate some form of non-coherent transmission in order to work well on all channels in $\mathcal{H}$ (see, e.g., \cite{o2017introduction}). 

Mathematically, we can formulate the problem as the optimization of the sum log-loss \eqref{eq:ce} over the channels in $\mathcal{H}$
\begin{align} \label{eq:joint}
\min_\theta \sum_{h\in\mathcal{H}} L_{h}(\theta).
\end{align}
In a manner similar to \eqref{eq:sgd}, problem \eqref{eq:joint} can be tackled via SGD as
\begin{align} \label{eq:joint_sgd}
\theta^{(i+1)} \leftarrow \theta^{(i)} - \kappa \nabla \sum_{h\in\mathcal{H}} \hat{L}_{h}(\theta^{(i)}),
\end{align}
for iterations $i=1,2,\ldots$, where $\kappa>0$ is a learning rate and the function $\hat{L}_{h}(\theta^{(i)})$ is computed as in \eqref{eq:empirical_loss}.

\subsection{Meta-Learning}
\label{subsec:maml}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\columnwidth]{fig_2.pdf}
    \caption{Meta-learning set-up via MAML: The goal is to find an initialization $\theta^{(0)}$ such that encoder and decoder parameters $\theta$ can be adapted to any channel with few SGD steps.}
    \label{fig:meta}
\end{figure}

While joint training obtains a common model $\theta$ for all channels in $\mathcal{H}$, meta-learning obtains a common initialization $\theta^{(0)}$, to be used for \emph{local training} as in Algorithm~\ref{alg:simple_ae}, for all channels in $\mathcal{H}$. As illustrated in Fig.~\ref{fig:meta}, the goal is to enable faster convergence, based on fewer iterations in Algorithm~\ref{alg:simple_ae}, to an effective solution for any channel related to those in $\mathcal{H}$. Therefore, ideally, meta-learning produces coherent encoding and decoding schemes more quickly, rather than providing optimized non-coherent solutions. 

As a notable example of meta-learning, MAML \cite{finn2017model} seeks for an initialization value $\theta^{(0)}$ that optimizes the problem
\begin{align} \label{eq:maml}
\min_{\theta^{(0)}}{L^\text{ML}} (\theta^{(0)}) = \sum_{h\in\mathcal{H}} L_{h}(\theta^{(0)}-\eta\nabla\hat{L}_{h}(\theta^{(0)})),
\end{align}
where the log-loss function $L_{h}(\cdot)$ and $\hat{L}_{h}(\cdot)$ are defined as in \eqref{eq:ce} and \eqref{eq:empirical_loss}, respectively. According to \eqref{eq:maml}, MAML aims to find an initialization value $\theta^{(0)}$ from which a single SGD update \eqref{eq:sgd} on each channel $h$ yields minimal log-loss. The key idea is that, if we succeed in finding an initialization point $\theta^{(0)}$ that yields a good solution for the channels in $\mathcal{H}$ after one SGD iteration, we can expect the initialization point $\theta^{(0)}$ to produce an effective autoencoder also for a new channel with only a small number of SGD iterations. 

Denoting as $U_h(\theta^{(0)}) = \theta^{(0)}-\eta\nabla\hat{L}_{h}(\theta^{(0)})$ the local updated vector for channel $h$, MAML tackles \eqref{eq:maml} via SGD through the update \eqref{eq:gd_ML}, which can be computed as
\begin{align} \label{eq:meta_update}
\nonumber
\theta^{(0, i+1)} &\leftarrow \theta^{(0,i)} - \kappa\sum_{h\in\mathcal{H}}(\mathbf{J}_{\theta^{(0)}}U_h(\theta^{(0,i)}))\nabla L_{h}(U_h(\theta^{(0,i)}))
\\
& \approx  \theta^{(0,i)} - \kappa \sum_{h\in\mathcal{H}} (I-\eta\nabla^2 \hat{L}_{h}(\theta^{(0,i)})) \nabla\hat{L}'_{h}(U_h(\theta^{(0,i)})),
\end{align}
for iterations $i=1,2,\ldots$, where $\mathbf{J}_{\theta^{(0)}}$ represents the Jacobian operation. The approximation in the last line is due to the estimation of the cross-entropy loss $L_{h}(\cdot)$ with the empirical loss $\hat{L}'_{h}(\cdot)$ obtained using $P$ i.i.d. samples $\mathcal{D}^{(i)'}=\{ m_j\sim p(m), w_j \sim \mathcal{CN}(0,N_0) \}_{j=1}^P$. The full algorithm is summarized in Algorithm~\ref{alg:ae_training}.


\begin{algorithm}[h] %!
\DontPrintSemicolon
\smallskip
\KwIn{meta-training channels $\mathcal{H} = \{ h_k \}_{k=1}^K$; number of samples per iteration $P$; step size hyperparameters $\eta$ and $\kappa$}
\KwOut{learned initial parameter vector $\theta^{(0)}$}
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
{\bf initialize} parameter vector $\theta^{(0,0)}$ \\
$i=0$ \\
\While{{\em not converged}}{
\For{{\em each meta-training channel $h\in\mathcal{H}$}}{
\vspace{0.05cm} compute local adaptation $U_h(\theta^{(0,i)}) = \theta^{(0,i)}-\eta\nabla\hat{L}_{h}(\theta^{(0,i)})$\\
}
update initialization parameter vector 
\vspace{-0.25cm}
\begin{align} \label{eq:gd_ML}
\theta^{(0,i+1)} \leftarrow \theta^{(0,i)} - \kappa \nabla L^\text{ML}(\theta^{(0,i)})
\end{align}
\\
\vspace{-0.4cm}
$i\leftarrow i+1$
}
\caption{Autoencoder-Based Meta-Learning}
\label{alg:ae_training}
\end{algorithm}
